Improving Dialogue State Tracking by Joint Slot Modeling

Dialogue state tracking models play an important role in a task-oriented dialogue system. However, most of them model the slot types conditionally independently given the input. We discover that it may cause the model to be confused by slot types that share the same data type. To mitigate this issue, we propose TripPy-MRF and TripPy-LSTM that models the slots jointly. Our results show that they are able to alleviate the confusion mentioned above, and they push the state-of-the-art on dataset MultiWoZ 2.1 from 58.7 to 61.3. Our implementation is available at https://github.com/CTinRay/Trippy-Joint.

==> sections/experiment.tex <==
Following the common practice of DST studies, we train and test our model on MultiWOZ  2.1 \cite{eric2019multiwoz}. There are 5 domains (train, restaurant,hotel, taxi, attraction) and 30 tracked slot types.

% We use the pre-trained BERT-base-uncased trans-former \cite{vaswani2017attention} as context encoder front-end.  This model has 12 hidden layers with 768 units and 12 self-attention heads each. The maximum  input  sequence  length  is  set  to  512 tokens  after  WordPiece  tokenization \cite{wu2016google}

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
 


\paragraph{Problem Statement}

Tracking  dialogue  states  is  the  core  component  to  ensure a robust manner in dialog systems.  In order to fulfill a user goal, a dialogue system must be capable of extracting meaning and intent from the user input, and be able to keep and up-date this information over the continuation of the dialog \cite{young2010hidden}. This task is called dialog state tracking (DST).  For example, in order to recommend a restaurant to a user, the systemn eeds to know their preferences in terms of price,location, etc. These concepts are encapsulated in an ontology, where dialogue domain (e.g., restaurant or hotel), slot (e.g., price range or location), and value (e.g. cheap or expensive) are defined. Solving this information extraction task is prerequisite for forming a belief over the dialog state

The  traditional  methods,  which  have been widely used in most commercial implementations, often  adopt  hand-crafted  rules  to  select  the  most  likely  result\cite{goddeau1996form}.   However,  these  rule-based  systems  are  prone  to frequent  errors  as  the  most  likely  result  is  not  always  the desired one\cite{williams2014web}.



In this survey, we first conduct a comprehensive study of the traditional as well as recent architectures and techniques used to model this task. We further transition to explore commonly used methods for Multi-domain dialog state tracking. Furthermore, we deep dive into benchmark data sets and state-of-the art models used in this task.



% \paragraph{Contribution-4 (Optional)}
% Lastly, in order to better understand
% the (zero-shot) ability of multi-lingual
% pretrained models
% in comprehending switching,
% we propose some probing experiments.
% Specifically, we try to understand what
% factors -- shared information between subwords
% or 



==> sections/modeling_setup.tex <==
\section{Datasets}
\label{sec:modeling}

\subsection{Benchmarking Pretrained Models}

% \subsection{Fine-tuning Strategies}

% \paragraph{Baselines}
% \begin{itemize}
%     \item Domain adaptive pretraining \newline \textit{(only for Hinglish ?)}
%     \item Representation Fusion
% \end{itemize}

% \paragraph{Ours}
% \begin{itemize}
%     \item Multi-task learning
%     \item Code-switched Language Modeling
%     \item Iterative Data Augmentation
% \end{itemize}

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\cite{williams-etal-2013-dialog} is the first benchmark for DST models. 
After that, \cite{henderson-etal-2014-second} proposed the DSTC2 dataset which includes more linguistic phenomena.
\cite{ramadan2018large} proposed MultiWoz, which is the first large scale human-human multi-domain task-oriented DST dataset.
Its successive versions \cite{eric2019multiwoz,zang-etal-2020-multiwoz} cleanse the noisy conversations in it.
Since then, it has become the standard DST benchmark dataset.

Early approaches for DST rely on a list candidate slot values \cite{mrksic-etal-2017-neural,Liu2017,ramadan-etal-2018-large,rastogi2017scalable}. 
Some recent approaches formulate it as a sequence generation task.
TRADE \cite{wu-etal-2019-transferable} and MA-DST \cite{kumar2020ma} generates slot values with a pointer generator with a copy mechanism.
SOM-DST \cite{kim-etal-2020-efficient} uses a BERT model to encode the dialogue. To improve the efficiency, the state from the previous turn instead of the whole dialogue history is fed into the model. 
SUMBT \cite{lee-etal-2019-sumbt} utilizes a BERT model \cite{devlin-etal-2019-bert} to encode both the dialogue history and candidate slot values.
In \cite{gao-etal-2019-dialog} they formulate DST as a question answering task.
DS-DST \cite{zhang-etal-2020-find} adopts a dual strategy: they predict slot values from candidates but also predict slot slot values by copying from the dialogue.
Trippy \cite{heck-etal-2020-trippy} predicts slot values by copying text span from three different sources.
In \cite{MehriDialoGLUE2020}, they improve the performance of Trippy by pre-training the BERT with multiple dialogue tasks.
Simple-TOD \cite{hosseini2020simple} and SOLOIST \cite{peng2020soloist} utilize GPT-2 for end-to-end slot value and response generation. 
In \cite{SHIYANG2020CoCoCC}, they investigate the generalization capability of DST models for unseen slot values.
MinTL \cite{lin2020mintl} augments data by substituting slot values in the utterances and modifying the syntax structure.


==> sections/results_discussion.tex <==
\section{Results \& Discussion}
\label{sec:results_discussion}

\input{emnlp2020-templates/tables/benchmarking}
\input{emnlp2020-templates/tables/pos}
% \input{emnlp2020-templates/tables/datasets_stats}


==> sections/trippy_section.tex <==

For replication of baseline, we picked TripPy: Triple copy strategy DST. The  model  expects  the  following  input  format to  perform  dialog  state  tracking. Let \textit{X={(U1,M1),...,(UT,MT)} } be  the  sequence  of turns that comprise a dialog of length \textit{T}. \textit{Ut} is the  user  utterance  at  turn \textit{t}, \textit{Mt} is  the  system utterance  that  precedes  the  user  utterance.   The task  of  the  model  is  (1)  to  determine  for  every turn whether any of the N domain-slot pairs in \textit{ S={S1,...,SN} }is present, (2) to predict the values for each \textit{Sn} and (3) to track the dialog state \textit{DSt} over the course of the dialog, i.e., for \textit{ t∈[1,T] }.We employ a triple-copy strategy to fill the slots.The intuition is that values are either explicitly ex-pressed by the user, that they are expressed by the system and referred to by the user via confirmation or rejection, or that they have been expressed earlier in the dialog as assignment to another domain-slot pair (co-reference). Each of these cases is handled by one of three copy mechanisms
 






